A test bed for measuring UAV servo reliability

Extant literature suggests minimal research in the area of system reliability of components used in the design of these UAS (Unmanned Air Systems), thus, subjecting UAS to critical failures that may pose a safety hazard to flight operations. The purpose of the study was to critically assess the reliability of a laboratory designed UAS component test-bed operated using real-world data collected from a Boeing Scan Eagle UAS aileron servo unit via a flight data recorder. The study hypothesized that the test-bed unit's replicating a UAS aileron servo motor's reliability, in terms of a base-line measured encoder output of commanded servo positions, will not be significantly different after double and triple periods of time for continuous operating cycles. Study adds to paucity of extant research on UAS reliability and recommends further studies on commercial UAS components reliability and time to failure.

==> 00-abstract.tex <==
\begin{abstract}
	\lettrine{T}{he} era of unmanned aviation is flourishing and advancing in leaps and bounds jumping over all challenges and obstacles. 
	% Within the contemporary timeframe, there has been tremendous improvements in research and development of unmanned aerial systems (UAS) in terms of applications in the broader aviation environment.
	Initial challenges in terms of design and applications of UAS\footnote{Unmanned Air Systems} are being surmounted with continuous data-driven improvements. However, extant literature suggests minimal research in the area of system reliability of components used in the design of these UAS. The issue escalates as COTS\footnote{Commercials Off the Shelf} are used with very minimal reliability  and operational life expectancy data
	In the absence of such functional integrity reliability analysis of components, UAS may be prone to critical failures that may pose a safety hazard.
	 % ( collisions) to human operators and physical infrastructure during flight operations especially beyond visual line of vision flights (BVLOS).	
	% The rationale for this study is further justified by the fact that many of the components used on UAS are COTS\footnote{Commercials Off the Shelf} with very minimal reliability  and operational life expectancy data. 
	To entertain this cause for servo motors as one crucial type of UAS used COTS, this study introduces a laboratory designed test-bed. The platform operates the servo to failure using the actual real-life service deployments. The exploited data was obtained from a servo unit used on the Boeing Insitu Scan Eagle UAS\textsuperscript{\textregistered} to control its ailerons.  The test-bed commands the servo and logs its actual movements along with the commanded positions. These logs were used to detect the discrepancy between the commanded and actual positions to give a statistical estimate about how long the servo will endure.

	% This study focuses on UAS servo components which have very limited reliability analysis and data within the operational environment.
	% Data extracted from a servo unit used on the Boeing Insitu Scan Eagle UAS to control its ailerons was used to provide a case-study for the introduced platform.
	The study shows a significant deterioration in the performance of the servo unit during in the lab experiment which carried out 3649 aileron positions over 364 servo-operation hours. Though this experiment did not investigate a particular servo-unit, it illustrates the contribution of the platform.
	% What were the significant findings? This is where you state the significant findings.
	% This study has significant research and policy implications. It can provide a data-driven framework and shape policies on reliability standards for UAS components. This framework is essential for regulatory agencies that have to certify UAS for commercial applications and especially BVLOS operations. It will also add up to the paucity of literature on the subject matter.
	This results has significant research and policy implications for regulatory bodies such as the FAA\footnote{Federal Aviation Administration} that has to certify UAS for commercial applications and especially BVLOS operations. It will add up to the paucity of literature on the subject matter and can provide relevant empirical data to assist in shaping policy on reliability standards for UAS designs.












	
	\begin{comment}
		\lettrine{T}{he} era of Unmanned aviation is flourishing and advancing in leaps and bounds jumping over all challenges and obstacles. One of the serious hinderances to the booming industry is the lack of sufficient reliability studies about the systems used on board these flying robots. Accordingly, this poses a threat to the safety and well-being of human communities as well as the loss of assets, especially in BLOS\footnote{Beyond Line Of Sight} flights. 
		The need for a reliable endurance investigation is emerging from the fact that many of the systems and components used on UAS\footnote{Unmanned Aerial System(s) [drones]}\footnote{Through out the paper, the term UAS is used interchangeably with UAV (Unmanned Air Vehicles)} are COTS\footnote{Commercials Off the Shelf} which comes with scarce information, if any, about its reliability and operation-life expectancy. This topic is of vital importance to regulatory organizations to consider legalizing commercial flights that are not in the field of the human operators' line of sight. 
Servos are one type of these crucial components used in UAS which lack thorough reliability evaluations. This study addresses this concern through a case study of the servo used on the Boeing Insitu ScanEagle\textsuperscript{\textregistered} to control its ailerons. To offer the expected information about the reliability of the components, a destructive test platform was sought. A test-bed was designed to operate a servo to failure using the actual commanded positions it operates to in its real-life service. The test-bed commands the servo and logs its actual movements along with the commanded positions. These logs are used to detect the discrepancy between the commanded and actual positions to give a statistical estimate about how long the servo will endure. Though the actual aircraft case-study servo type was not used in the experiments, the test-bed can operate on any servo-motor.

	\end{comment}
	
	
\end{abstract}

==> 04-dataPreparation.tex <==
\section{Data Preparation}
Boeing Insitu ScanEagle\textsuperscript{\textregistered} is equipped with a Horizon MicroPilot\textsuperscript{\textregistered}\footnote{url{https://www.micropilot.com}}. Flight data is downloaded after each flight using a MicroPilot software product called Logviewer.

The study's used data file is 7854 entires representing data points collected from a point-to-point flight. The aircraft's autopilot samples data at the rate of 5 samples per seconds. This means that the data covers about 26.2 mins flight. The maximum altitude reached in the recorded flight is 2267 feet. The FDR saves the aileron servo postion in measurement units called 'fine servo units'. These units range between -32,767 and +32,767 and has to be converted to rotational degrees given that the servo rotation range is $[0\textsuperscript{\textdegree}, 180\textsuperscript{\textdegree}]$.

An FDR log file was used to statistically study the positions of the servo during flight. The results of this study is shown in Table~\ref{tab:neg_stat} for the negative aileron angles, and Table~\ref{tab:pos_stat} for the positive aileron angles. As shown, the number of positive aileron positions exceed the number of negative positions, which is expected because negative position acts as an aid for the positive position on the opposite side aileron in severe maneuvers. Figures~\ref{fig:histo_pos_postions}, and~\ref{fig:histo_all_postions}, show the frequencies of the angles in the FDR file.
% Box-plot shown in Figure~\ref{fig:box_plot} show the confidence interval of the positions in the FDR file.
% The outliers are also shown in the figure.
% The 50\% confidence interval shows that maximum and minimum positions are $9.84^\circ$, and $19.69^\circ$ respectively, while for the negative positions are $-11.25^\circ$ and $-5.63^\circ$ respectively.]
The data has a 50\% confidence interval [$9.84^\circ$, $19.69^\circ$] for the positive positions, and [$-11.25^\circ$, $-5.63^\circ$] for the negative positions, based on the data median in both data groups (refer to Figure~\ref{fig:surfaceServoSys} for angle sign).

A list of positions ( positive and negative) was prepared based on FDR data output to reflect the angles that the servo operate in real life and their frequencies. This list took into consideration the real-life servo operation and represented this in the number of times each position appear in the list. Table~\ref{tab:position} depicts a sample of the prepared list based on the FDR file.


% \begin{figure}
% \includegraphics[width=.49\textwidth, height=.98\textheight]{./img/{NegativeAnglesPlots}.pdf}
% \caption{Aileron Negative Positions Boxplot \& Histogram. \label{fig:neg_plot} }
% \end{figure}
%
% \begin{figure}
% \includegraphics[width=.49\textwidth, height=.98\textheight]{./img/{PositiveAnglesPlots}.pdf}
% \caption{Aileron Positive Positions Boxplot \& Histogram.\label{fig:pos_plot}}
% \end{figure}

% \begin{figure}
% \subfloat[\normalsize Logged Aileron Negative Positions Histogram.]{\includegraphics[width=.49\textwidth, height=.45\textheight]{./img/{NegativeAnglesPlots}.pdf}
% \label{fig:neg_plot}}
% \\
% \subfloat[\normalsize Logged Aileron Positive Positions Histogram.]{\includegraphics[width=.49\textwidth, height=.45\textheight]{./img/{PositiveAnglesPlots}.pdf}
% \label{fig:pos_plot}}
% \caption{Logged Aileron Positions Boxplot Histogram.}
% \end{figure}


% \begin{figure}
% \subfloat[\normalsize Logged Aileron Negative Positions Histogram.]{\includegraphics[width=.49\textwidth, height=.45\textheight]{./img/{NegativeAnglesPlots}.pdf}
% \label{fig:neg_plot}}
% \\
% \subfloat[\normalsize Logged Aileron Positive Positions Histogram.]{\includegraphics[width=.49\textwidth, height=.45\textheight]{./img/{PositiveAnglesPlots}.pdf}
% \label{fig:pos_plot}}
% \caption{Logged Aileron Positions Boxplot Histogram.}
% \end{figure}


% \begin{table}
% \centering
% \small
%   \caption{Positions Statistical Description}
%   \label{tab:stat}
%   \begin{tabular}{llrlr}
% 	 \multicolumn{1}{l} {}& \multicolumn{2} {c} {\bfseries Negative Positions} & \multicolumn{2} {c} {\bfseries Positive Positions}\\
%     \toprule
%     \textbf{N} 						& Valid 	& 1095		& Valid		& 6557		\\
%       								& Missing 	& 0			& Missing	& 0			\\
% 	\textbf{Mean}\hspace{1cm}					&			& -11.6022	&			& 16.2681	\\
% 	\textbf{Std. Error of Mean} 	&			& .28664	&			& .13087	\\
% 	\textbf{Median}					&			& -11.2503	& 			& 14.0629	\\
% 	\textbf{Std. Deviation}			&			& 9.48505	&			& 10.59699	\\
% 	\textbf{Variance}				&			& 89.966	&			& 112.296	\\
% 	\textbf{Skewness}				&			& -2.701	& 			& 1.912 	\\
% 	\textbf{Std. Error of Skewness}\hspace{1cm} &			& .074		&			& .030		\\
% 	\textbf{Kurtosis}				&			& 10.336	&			& 5.957		\\
% 	\textbf{Std. Error of Kurtosis}	&			& .148		&			& .060		\\
% 	\textbf{Range}					& 			& 73.13		&			& 87.19		\\
% 	\textbf{Minimum}				&			& -74.53	&			& 1.41		\\
% 	\textbf{Maximum}				&			& -1.41		& 			& 88.60		\\
% 	\textbf{Percentiles} 			& 25		& -11.2503	& 25		& 9.8441	\\
% 									& 50		& -11.2503	& 50		& 14.0629	\\
% 									& 75		& -5.6252	& 75		& 19.6881	\\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table}
\centering
  \caption{Positions Statistical Description}
  \label{tab:neg_stat}
  \begin{tabular}{llr}
    \toprule
    \textbf{N} 						& Valid 	& 1095		\\
      								& Missing 	& 0			\\
	\textbf{Mean}\hspace{1cm}					&			\\
	\textbf{Std. Error of Mean} 	&			& .28664	\\
	\textbf{Median}					&			& -11.2503	\\
	\textbf{Std. Deviation}			&			& 9.48505	\\
	\textbf{Variance}				&			& 89.966	\\
	\textbf{Skewness}				&			& -2.701	\\
	\textbf{Std. Error of Skewness} &			& .074		\\
	\textbf{Kurtosis}				&			& 10.336	\\
	\textbf{Std. Error of Kurtosis}	&			& .148		\\
	\textbf{Range}					& 			& 73.13		\\
	\textbf{Minimum}				&			& -74.53	\\
	\textbf{Maximum}				&			& -1.41		\\
	\textbf{Percentiles} 			& 25		& -11.2503	\\
									& 50		& -11.2503	\\
									& 75		& -5.6252	\\
    \bottomrule
  \end{tabular}
\end{table}

\begin{table}
	\centering
  \caption{Negative Positions Statistical Description}
  \label{tab:pos_stat}
  \begin{tabular}{llr}
    \toprule
	\textbf{N} 								& Valid		& 6557		\\
											& Missing	& 0			\\
	\textbf{Mean}							&			& 16.2681	\\
	\textbf{Std. Error of Mean}				&			& .13087	\\
	\textbf{Median}							& 			& 14.0629	\\
	\textbf{Std. Deviation}					&			& 10.59699	\\
	\textbf{Variance}						&			& 112.296	\\
	\textbf{Skewness}						& 			& 1.912 	\\
	\textbf{Std. Error of Skewness}			&			& .030		\\
	\textbf{Kurtosis}						&			& 5.957		\\
	\textbf{Std. Error of Kurtosis}			&			& .060		\\
	\textbf{Range}							&			& 87.19		\\
	\textbf{Minimum}						&			& 1.41		\\
	\textbf{Maximum}						& 			& 88.60		\\
	\textbf{Percentiles} 					& 25		& 9.8441	\\
											& 50		& 14.0629	\\
											& 75		& 19.6881	\\
    \bottomrule
  \end{tabular}
\end{table}

% \begin{figure}
% 	\centering
% \includegraphics[width=.48\textwidth, height=.45\textheight]{./img/{box_plot}.pdf}
% \caption{\label{fig:box_plot}Logged Aileron Positions Box-Plot.}
% \end{figure}


\begin{table}
	\centering
% \fontsize{8pt}{5pt}\selectfont
  \caption{Commanded Positions}
  \label{tab:position}
  \begin{tabular}{cccccccccccccccccccccccc}
    \toprule

4	& -11	& 13	& -11 	& 32	& 15	& 7		& 17	& 23	& 14	%\\
3	& 11	& 11	& 11	& 10	& 17	& -1	& -11	& 18	& 6		\\
25	& -10	& 25	& 20	& 11	& 10	& 7		& -24	& 7		& 37	%\\
8	& 14	& -18	& -14	& 10	& 11	& -4	& 17	& 35	& 6		\\
3	& 14	& 28	& 17	& 34	& -6	& 11	& -30	& 4		& 13	%\\
17	& 21	& 11	& 15	& -20	& -1	& 24	& 20	& 6		& -11	\\
14	& 13	& 24	& -25	& 21	& 8		& -13	& 23	& 14	& -15	%\\
3	& 14	& 17	& 30	& 31	& 15	& -28	& 14	& -11	& 15	\\
1	& 27	& 13	& -8	& 8		& -3	& -7	& 10	& 8		& 10	%\\
7	& 18	& 27	& 14	& 20	& 8		& 4		& 13	& 15	& -17	\\
23	& -11	& -3	& 18	& 8		& 20	& 13	& -21	& 6		& -27	%\\
-23	& 21	& 15	& 13	& 10	& 13	& 28	& 15	& 7		&		\\
    \bottomrule
  \end{tabular}
\end{table}

% \begin{figure}
% % \begin{sidewaysfigure}
% \centering
% \subfloat[Training error for 1 second predictions.]{\includegraphics[width=.48\textwidth, height=.20\textheight]{./img/{cost_fun_all_art_1}.pdf}
% \label{fig:art_all_cost_1sec}}
% % \quad
% % \\
% \subfloat[Training error for 5 second predictions.]{\includegraphics[width=.48\textwidth, height=.20\textheight]{./img/{cost_fun_all_art_5}.pdf}
% \label{fig:art_all_cost_5sec}}
% \\
% \subfloat[Training error for 10 second predictions.]{\includegraphics[width=.48\textwidth, height=.20\textheight]{./img/{cost_fun_all_art_10}.pdf}
% \label{fig:art_all_cost_10sec}}
% % \quad
% % \\
% \subfloat[Training error for 20 second predictions.]{\includegraphics[width=.48\textwidth, height=.20\textheight]{./img/{cost_fun_all_art_20}.pdf}
% \label{fig:art_all_cost_20sec}}
% \caption{Mean squared error during the training process for the three architectures predicting vibration in 1, 5, 10, and 20 seconds in the future.}
% \label{fig:art_all_costs}
% % \end{sidewaysfigure}
% \end{figure}

==> 09-appedices.tex <==
\begin{appendices}
\section{Dataset Outputs}

\begin{table}[h]
	\tiny
	\centering
  \caption{Tests of Within-Subjects Effects}
  \label{}
  \begin{tabular}{llcccc}
	\multicolumn{6}{l}{Measure: MEASURE\_1} \\
	\hline
	\multicolumn{1}{l}{\bfseries Source} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\bfseries \makecell{Type III \\ Sum \\ of Squares}} & \multicolumn{1}{c}{\bfseries df} & \multicolumn{1}{c}{\bfseries  \makecell{Mean \\ Square} } & \multicolumn{1}{c}{\bfseries F} \\
    \toprule
	\multirow{4}{*}{Cycle}			& Sphericity Assumed	& 2				& 2			& 1836.126	& 21.019	\\
		 							& Greenhouse-Geisser	& 3672.252		& 1.354		& 2712.042	& 21.019	\\
									& Huynh-Feldt			& 3672.252		& 1.380		& 2660.917	& 21.019	\\
									& Lower-bound			& 3672.252		& 1.000		& 2660.917	& 3672.252	\\
	\hline
	\multirow{4}{*}{\makecell{Error\\(Cycle)}}	& Sphericity Assumed	& 8211.475		& 94		& 87.356	& 	\\
		 							& Greenhouse-Geisser	& 8211.475		& 63.641	& 129.029	& 	\\
									& Huynh-Feldt			& 8211.475		& 64.863	& 126.597	& 	\\
									& Lower-bound			& 8211.475		& 47.000	& 174.712	& 	\\
    \bottomrule
  \end{tabular}
\end{table}



\begin{table}[h]
	\footnotesize
	\centering
  \caption{Tests of Within-Subjects Effects}
  \label{}
  \begin{tabular}{llcc}
	\multicolumn{4}{l}{Measure: MEASURE\_1} \\
	\hline
	\multicolumn{1}{l}{\bfseries Source} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\bfseries \makecell{Sig.}} & \multicolumn{1}{c}{\bfseries  Partial $\eta^2$} \\
    \toprule	
	
	\multirow{4}{*}{Cycle}			& Sphericity Assumed	& 0.000		& 0.309	\\
		 							& Greenhouse-Geisser	& 0.000		& 0.309	\\
									& Huynh-Feldt			& 0.000		& 0.309	\\
									& Lower-bound			& 0.000		& 0.309	\\
	\hline
	\multirow{4}{*}{\makecell{Error\\(Cycle)}}	& Sphericity Assumed 	\\
												& Greenhouse-Geisser	\\
												& Huynh-Feldt			\\
												& Lower-bound			\\
    \bottomrule
	
    \bottomrule
  \end{tabular}
\end{table}	
	
	
	
	
	
	
\begin{table}[h]
	\tiny
	\centering
  \caption{Tests of Within-Subjects Contrasts}
  \label{}
  \begin{tabular}{llcccc}
	\multicolumn{6}{l}{Measure: MEASURE\_1} \\
	\hline
	\multicolumn{1}{l}{\bfseries Source} & \multicolumn{1}{c}{Cycle} & \multicolumn{1}{c}{\bfseries \makecell{Type III \\ Sum \\ of Squares}} & \multicolumn{1}{c}{\bfseries df} & \multicolumn{1}{c}{\bfseries  \makecell{Mean \\ Square} } & \multicolumn{1}{c}{\bfseries F} \\
    \toprule
	\multirow{2}{*}{Cycle}			& Level 1 vs. Level 2	& 1502.707		& 1		& 1502.707	& 27.491	\\
		 							& Level 2 vs. Level 3	& 2191.117		& 1		& 2191.117	& 9.775		\\
	\hline
	\multirow{2}{*}{Cycle}			& Level 1 vs. Level 2	& 2569.092		& 47		& 54.662	\\
		 							& Level 2 vs. Level 3	& 10535.264		& 47		& 224.155	\\
    \bottomrule
  \end{tabular}
\end{table}



\begin{table}[h]
	\footnotesize
	\centering
  \caption{Tests of Within-Subjects Contrasts}
  \label{}
  \begin{tabular}{llcc}
	\multicolumn{4}{l}{Measure: MEASURE\_1} \\
	\hline
	\multicolumn{1}{l}{\bfseries Source} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\bfseries \makecell{Sig.}} & \multicolumn{1}{c}{\bfseries  Partial $\eta^2$ } \\
    \toprule
	\multirow{2}{*}{Cycle}			& Level 1 vs. Level 2	& 0.000		& 0.369 \\
		 							& Level 2 vs. Level 3	& 0.003		& 0.172	\\
	\hline
	\multirow{2}{*}{Cycle}			& Level 1 vs. Level 2	\\
		 							& Level 2 vs. Level 3	\\
    \bottomrule
  \end{tabular}
\end{table}




\begin{table}[h]
	\tiny
	\centering
  \caption{Tests of Between-Subjects Effects}
  \label{}
  \begin{tabular}{lcccccc}
	\multicolumn{7}{l}{Measure: MEASURE\_1} \\
	\multicolumn{7}{l}{Transformed Variable: Average} \\
	\hline
	\multicolumn{1}{l}{\bfseries Source} & \multicolumn{1}{c}{\bfseries \makecell{Type III \\ Sum \\ of Squares}} & \multicolumn{1}{c}{\bfseries df} & \multicolumn{1}{c}{\bfseries  \makecell{Mean \\ Square} } & \multicolumn{1}{c}{\bfseries F} & \multicolumn{1}{c}{Cycle} & \multicolumn{1}{c}{Partial $\eta^2$} \\
    \toprule
	Intercept	& 174630.599	& 1		& 174630.599	& 70.761	& 0.000		& 0.601	\\
	Error		& 115991.001	& 47	& 47	& 2467.894	\\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[h]
	\tiny
	\centering
  \caption{Parameter Estimates}
  \label{}
  \begin{tabular}{llcccc}
	\multicolumn{1}{l}{\bfseries Dependent Variable} & \multicolumn{1}{c}{\bfseries Parameter} & \multicolumn{1}{c}{\bfseries B} & \multicolumn{1}{c}{\bfseries  Std. Error } & \multicolumn{1}{c}{\bfseries t} & \multicolumn{1}{c}{Sig.}	\\
    \toprule
	Cycle\_1\_130	& Intercept		& 54.335	& 6.468		& 8.400		& 0.000	\\
	Trial\_2		& Intercept		& 59.930	& 7.261		& 8.253		& 0.000	\\
	Cycle\_3\_390	& Intercept		& 66.686	& 7.958		& 8.380		& 0.000	\\
    \bottomrule
  \end{tabular}
\end{table}


\begin{table}[h]
	\tiny
	\centering
  \caption{Parameter Estimates}
  \label{}
  \begin{tabular}{llccc}
	&	& 	 \multicolumn{2}{c}{\bfseries $95\%$ Confidence Interval}	&	\\
	\cline{3-4}
	\multicolumn{1}{l}{\bfseries Dependent Variable} & \multicolumn{1}{c}{\bfseries Parameter} & \multicolumn{1}{c}{\bfseries \makecell{Lower \\ Bound}} & \multicolumn{1}{c}{\bfseries \makecell{Upper \\ Bound} } & \multicolumn{1}{c}{\bfseries  Partial $\eta^2$ } 	\\
    \toprule
	Cycle\_1\_130	& Intercept		& 41.323	& 67.347	& 0.600		\\
	Trial\_2		& Intercept		& 45.322	& 74.538	& 0.592		\\
	Cycle\_3\_390	& Intercept		& 50.678	& 82.695	& 0.599		\\
    \bottomrule
  \end{tabular}
\end{table}



\begin{table}[h]
	\footnotesize
	\centering
  \caption{Parameter Estimates}
  \label{}
  \begin{tabular}{lcccc}
	\multicolumn{5}{l}{Estimates}\\
	\multicolumn{5}{l}{Measure: MEASURE\_1} \\
	&	& 	 & \multicolumn{2}{c}{\bfseries $95\%$ Confidence Interval}		\\
	\cline{4-5}
	\multicolumn{1}{l}{\bfseries Cycle} & \multicolumn{1}{c}{\bfseries Mean} & \multicolumn{1}{c}{\bfseries std. Error} & \multicolumn{1}{c}{\bfseries \makecell{Lower \\ Bound}} & \multicolumn{1}{c}{\bfseries \makecell{Upper \\ Bound}} \\
    \toprule
	1	& 54.335	& 6.468		& 41.323	& 67.347	\\
	2	& 59.930	& 7.261		& 45.322	& 74.538	\\
	3	& 66.686	& 7.958		& 50.678	& 82.695	\\
    \bottomrule
  \end{tabular}
\end{table}




\begin{table}[h]
	\tiny
	\centering
  \caption{Pairwise Comparisons}
  \label{}
  \begin{tabular}{llccccc}
	\multicolumn{7}{l}{Measure: MEASURE\_1} \\
		&	& \multicolumn{1}{c}{\bfseries \makecell{Mean \\ Difference}}	& 	&	& \multicolumn{2}{c}{\bfseries \makecell{$95\%$ Confidence Interval \\ for Difference\textsuperscript{b} } }	\\
	\cline{6-7}
	\multicolumn{1}{l}{\bfseries (I) Cycle} & \multicolumn{1}{l}{\bfseries (J) Cycle} & \multicolumn{1}{c}{\bfseries (I-J)} & \multicolumn{1}{c}{\bfseries std. Error}  & \multicolumn{1}{c}{\bfseries Sig.\textsuperscript{b}} & \multicolumn{1}{c}{\bfseries \makecell{Lower \\ Bound}} & \multicolumn{1}{c}{\bfseries \makecell{Upper \\ Bound}} \\
    \toprule
	\multirow{2}{*}{1}	& 2		& -5.595\textsuperscript{*}		& 1.067		& 0.000		& -8.245	& -2.946	\\
						& 3		& -12.352\textsuperscript{*}	& 0.000		& 2.261		& -17.964	& -6.739	\\
	\hline
	\multirow{2}{*}{2}	& 1		& -5.595\textsuperscript{*}		& 1.067		& 0.000		& 2.946		& 8.245		\\
						& 3		& -6.756*\textsuperscript{*}	& 2.261		& 0.000		& -12.121	& -1.391	\\
	\hline
	\multirow{2}{*}{2}	& 1		& 12.352\textsuperscript{*}		& 2.261		& 0.000		& 6.739		& 17.964	\\
						& 2		& 6.756*\textsuperscript{*}		& 2.261		& 2.161		& 1.391		& 12.121	\\
    \bottomrule
	\multicolumn{7}{l}{Based on estimated marginal means}							\\
	\multicolumn{7}{l}{*. The mean difference is significant at the .05 level.}		\\
	\multicolumn{7}{l}{b. Adjustment for multiple comparisons: Bonferroni.}			\\
  \end{tabular}
\end{table}




\begin{table}[h]
	\tiny
	\centering
  \caption{Pairwise Comparisons}
  \label{}
  \begin{tabular}{lcccccc}
	\multicolumn{7}{l}{Measure: MEASURE\_1} \\
		&	& 	& Hypothesis	&	&	& Partial\\
	\multicolumn{1}{l}{\bfseries Value} & \multicolumn{1}{l}{\bfseries F} & \multicolumn{1}{c}{\bfseries df} & \multicolumn{1}{c}{\bfseries Error df}  & \multicolumn{1}{c}{\bfseries Sig} & & \multicolumn{1}{c}{\bfseries $\eta^2$} \\
    \toprule
	Pillai's trace		& 0.479		& 21.148	& 2.000		& 46.000	& .000		& 0.479		\\
	Wilks' lambda		& 0.521		& 21.148	& 2.000		& 46.000	& .000		& 0.479		\\
	Hotelling's trace	& 0.919		& 21.148	& 2.000		& 46.000	& 0.000		& 0.479		\\
	Roy's largest root	& 0.919		& 21.148	& 2.000		& 46.000	& 0.000		& 0.479		\\
    \bottomrule
  \end{tabular}
\end{table}

\end{appendices}
